GSVNet: Guided Spatially-Varying Convolution for Fast Semantic Segmentation on Video

This paper addresses fast semantic segmentation on video.Video segmentation often calls for real-time, or even fasterthan real-time, processing. One common recipe for conserving computation arising from feature extraction is to propagate features of few selected keyframes. However, recent advances in fast image segmentation make these solutions less attractive. To leverage fast image segmentation for furthering video segmentation, we propose a simple yet efficient propagation framework. Specifically, we perform lightweight flow estimation in 1/8-downscaled image space for temporal warping in segmentation outpace space. Moreover, we introduce a guided spatially-varying convolution for fusing segmentations derived from the previous and current frames, to mitigate propagation error and enable lightweight feature extraction on non-keyframes. Experimental results on Cityscapes and CamVid show that our scheme achieves the state-of-the-art accuracy-throughput trade-off on video segmentation.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> figs/acc_thr_fig.tex <==
    \begin{figure}[t]
        %\captionsetup{textfont=normalfont}
        \begin{tikzpicture}
            %\centering
            \begin{axis}[
                name=axis1,
                yshift=4.5cm,
                height=4cm,width=8.5cm,
                xlabel={Throughput (FPS)},
                ylabel={Avg. mIoU ($\%$)},
                ylabel style={at={(axis description cs:0.05,0.5)}},
                xlabel style={at={(axis description cs:0.5,0.0)}},
                xmin=30, xmax=160,
                ymin=68, ymax=76,
                line width=1.0pt,
                mark size=2.0pt,
                xtick={30, 40, 50, 60, 70, 80, 90, 100, 110, 120, 130, 140,150,160},
                xmajorgrids,
                ytick={68, 70, 72, 74, 76},
                ymajorgrids,
                %legend pos=south west,
                legend style={at={(-0.1, 1.5)},anchor=north west, legend  columns =2, draw=none,cells={align=left}},
                legend cell align={left},
                %/tikz/every even column/.append style={column sep=1 cm}},
                grid style={solid, gray},
                %title={\MakeLabel{suba} Avg. mIoU vs. throughput},
            ]
            
            \addplot[
                color=cyan,
                mark=square,
                dashed,
                every mark/.append style={solid},
                ]
                coordinates { (61,73.7)(98.5,72.9)(123.4,72.0)(140,71.2)(153,70.3)
                };
            \addlegendentry{Ours-BN-R18 (0.75)}
            \addplot[
                color=green2,
                mark=square,
                dashed,
                every mark/.append style={solid},
                ]
                %coordinates {(105,69)};
                %72.7,71.7,71,70.5,70.1
                coordinates {(37,75.2)(64.5,74.2)(85.4,73.2)(101,72.3)(115,71.4)};
            \addlegendentry{Ours-BN-R18 (1.0)}
            
            %ours with swnet
            \addplot[
                color=blue,
                mark=*,
                ]
                coordinates { (63.2,74.4)(100,73.6)(125,72.6)(142,71.8)(155,70.9)
                };
            \addlegendentry{Ours-SN-R18 (0.75)}
            \addplot[
                color=red,
                %dashed,
                %every mark/.append style={solid},
                mark=*,
                ]
                coordinates {(37,74.6)(64.5,74.1)(85.4,73.4)(101,72.7)(115,71.9)};
            \addlegendentry{Ours-SN-R18 (1.0)}
            \end{axis}
            
            \begin{axis}[
                name=axis2,
                %at={(ax1.south east)},
                height=4cm,width=8.5cm,
                xlabel={Throughput (FPS)},
                ylabel={Min. mIoU ($\%$)},
                ylabel style={at={(axis description cs:0.05,0.5)}},
                xlabel style={at={(axis description cs:0.5,0.0)}},
                xmin=30, xmax=160,
                ymin=66, ymax=76,
                line width=1.0pt,
                mark size=2.0pt,
                xtick={30, 40, 50, 60, 70, 80, 90, 100, 110, 120, 130, 140,150,160},
                xmajorgrids,
                ytick={66, 68, 70, 72, 74, 76},
                ymajorgrids,
                %legend pos=south west,
                legend style={at={(-0.1, 1.5)},anchor=north west, legend  columns =2, draw=none},
                %/tikz/every even column/.append style={column sep=1 cm}},
                grid style={solid, gray},
                %title={\MakeLabel{subb} Min. mIoU vs. throughput},
            ]
            
            \addplot[
                color=cyan,
                mark=square,
                dashed,
                every mark/.append style={solid},
                ]
                coordinates { (61,73.7)(98.5,72.1)(123.4,70.5)(140,68.8)(153,67.1)
                };
            \addplot[
                color=green2,
                mark=square,
                dashed,
                every mark/.append style={solid},
                ]
                %coordinates {(105,69)};
                %72.7,71.7,71,70.5,70.1
                coordinates {(37,75.2)(64.5,73.3)(85.4,71.4)(101,69.8)(115,68.0)};
            %ours with swnet
            \addplot[
                color=blue,
                mark=*,
                ]
                coordinates { (63.2,74.4)(100,72.9)(125,70.7)(142,69.6)(155,67.7)
                };
            \addplot[
                color=red,
                %dashed,
                %every mark/.append style={solid},
                mark=*,
                ]
                coordinates {(37,74.6)(64.5,73.6)(85.4,72.0)(101,70.7)(115,69.1)};
            \end{axis}
            \node [below= 1.2cm] at (axis1.south) {\MakeLabel{subb}};
            \node [below= 1.2cm] at (axis2.south) {\MakeLabel{suba}};
            
        \end{tikzpicture}
        \caption{Comparison of accuracy-throughput curves.}
        \label{fig:keyframe_com}
    \end{figure}

==> figs/acc_thr_fig_cmp.tex <==
    \begin{figure}[t]
        %\captionsetup{textfont=normalfont}
        \begin{tikzpicture}
            %\centering
            \begin{axis}[
                name=axis1,
                yshift=4.5cm,
                height=4cm,width=8.5cm,
                xlabel={Throughput (FPS)},
                ylabel={Avg. mIoU ($\%$)},
                ylabel style={at={(axis description cs:0.05,0.5)}},
                xlabel style={at={(axis description cs:0.5,0.0)}},
                xmin=30, xmax=160,
                ymin=66, ymax=76,
                line width=1.0pt,
                mark size=2.0pt,
                xtick={30, 40, 50, 60, 70, 80, 90, 100, 110, 120, 130, 140,150,160},
                xmajorgrids,
                ytick={66, 68, 70, 72, 74, 76},
                ymajorgrids,
                %legend pos=south west,
                legend style={at={(-0.125, 1.7)},anchor=north west, legend  columns =3, draw=none,cells={align=left}},
                legend cell align={left},
                %/tikz/every even column/.append style={column sep=1 cm}},
                grid style={solid, gray},
                %title={\MakeLabel{suba} Avg. mIoU vs. throughput},
            ]
            
            \addplot[
                color=cyan,
                mark=square*,
                ]
                coordinates { (61,73.7)(98.5,72.9)(123.4,72.0)(140,71.2)(153,70.3)
                };
            \addlegendentry{Ours-BiSeNet-R18}
            \addplot[
                color=green2,
                mark=triangle,
                ]
                %coordinates {(105,69)};
                %72.7,71.7,71,70.5,70.1
                coordinates {(61,72.7)(58.8,71.7)(58.1,71)(57.4,70.5)(57.1,70.1)};
            \addlegendentry{A-X39}
            %\addplot[
            %    color=black,
            %    mark=triangle*,
            %    ]%(61,73.8)
            %coordinates{(61,68.6)(63.9,69.3)(64.6,69.3)(65.0,69.1)(65.3,68.8)};
            %\addlegendentry{A-X39}
            \addplot[
                color=black,
                mark=diamond*,
                ]%(61,73.8)
             %coordinates{(123.5,68.6)};
                coordinates {(105,69)};
            \addlegendentry{BiSeNet-X39}
            
            %ours with swnet
            \addplot[
                color=blue,
                mark=*,
                ]
                coordinates { (63.2,74.4)(100,73.6)(125,72.6)(142,71.8)(155,70.9)
                };
            \addlegendentry{Ours-SwiftNet-R18}
            \addplot[
                color=red,
                dashed,
                every mark/.append style={solid},
                mark=square,
                ]
                coordinates {(37,75.1)(61,73.8)(90,69.3)(131,68.9)};
            \addlegendentry{BiSeNet-R18}
            \addplot[
                color=purple1,
                dashed,
                every mark/.append style={solid},
                mark=o,
                ]
                %96 is not sure
                coordinates {(39.3,74.6)(63.2,74.4)(92,70.9)(134,68.7)};
            \addlegendentry{SwiftNet-R18}
            \addplot[
                color=purple2,
                every mark/.append style={solid},
                mark=x,
                ]
                coordinates {(108.7,67.3)};
            \addlegendentry{EDANet}
            \addplot[
                color=orange,
                every mark/.append style={solid},
                mark=star,
                ]
                coordinates {(123.5,68.6)};
            \addlegendentry{Fast-SCNN}
            %\addplot[
            %    color=purple2,
            %    dashed,
            %    every mark/.append style={solid},
            %    mark=diamond*,
            %    ]
            %    coordinates {};
            %\addlegendentry{ERFNet}
            
            \end{axis}
            
            \begin{axis}[
                name=axis2,
                %at={(ax1.south east)},
                height=4cm,width=8.5cm,
                xlabel={Throughput (FPS)},
                ylabel={Min. mIoU ($\%$)},
                ylabel style={at={(axis description cs:0.05,0.5)}},
                xlabel style={at={(axis description cs:0.5,0.0)}},
                xmin=30, xmax=160,
                ymin=66, ymax=76,
                line width=1.0pt,
                mark size=2.0pt,
                xtick={30, 40, 50, 60, 70, 80, 90, 100, 110, 120, 130, 140,150,160},
                xmajorgrids,
                ytick={66, 68, 70, 72, 74, 76},
                ymajorgrids,
                %legend pos=south west,
                legend style={at={(-0.1, 1.6)},anchor=north west, legend  columns =3, draw=none},
                %/tikz/every even column/.append style={column sep=1 cm}},
                grid style={solid, gray},
                %title={\MakeLabel{subb} Min. mIoU vs. throughput},
            ]
            
            \addplot[
                color=cyan,
                mark=square*,
                ]
                coordinates { (61,73.7)(98.5,72.1)(123.4,70.5)(140,68.8)(153,67.1)
                };
            %72.7,70.9,69.8,69.1,68.5
            \addplot[
                color=green2,
                mark=triangle,
                ]
                coordinates {(61,72.7)(58.8,70.9)(58.1,69.8)(57.4,69.1)(57.1,68.5)
                };
            %\addplot[
            %    color=black,
            %    mark=triangle*,
            %    ]%(61,73.8)
                %coordinates{(61,68.6)(63.9,68.6)(64.6,68.6)(65.0,68.6)(65.3,68.5)};
            \addplot[
                color=black,
                mark=diamond*,
                ]%(61,73.8)
             %coordinates{(123.5,68.6)};
                coordinates {(105,69)};
            %ours with swnet
            \addplot[
                color=blue,
                mark=*,
                ]
                coordinates { (63.2,74.4)(100,72.9)(125,70.7)(142,69.6)(155,67.7)
                };
            \addplot[
                color=red,
                dashed,
                every mark/.append style={solid},
                mark=square,
                ]
                coordinates {(37,75.1)(61,73.8)(90,69.3)(131,68.9)};
            \addplot[
                color=purple1,
                dashed,
                every mark/.append style={solid},
                mark=o,
                ]
                coordinates {(39.3,74.6)(63.2,74.4)(92,70.9)(134,68.7)};
            \addplot[
                color=purple2,
                every mark/.append style={solid},
                mark=x,
                ]
                coordinates {(108.7,67.3)};
            \addplot[
                color=orange,
                every mark/.append style={solid},
                mark=star,
                ]
                coordinates {(123.5,68.6)};
            \end{axis}
            \node [below= 1.2cm] at (axis1.south) {\MakeLabel{subb}};
            \node [below= 1.2cm] at (axis2.south) {\MakeLabel{suba}};
            
        \end{tikzpicture}
        \caption{Comparison of accuracy-throughput curves evaluated on Cityscapes validation set.
        %To explore the trade-off trend of image-based methods, we take three variants based on different input scales containing $\{1.0, 0.75, 0.6, 0.5\}$ of BiSeNet~\cite{bisenet} and SwiftNet~\cite{swiftnet} for comparison.
        The dashed lines correspond to image-based methods, where different accuracy-throughput trade-offs are achieved by adapting the input resolution with factors \{1, 0.75, 0.6, 0.5\}. EDANet, Fast-SCNN, and BiSeNet-X39 have an input scaling factor of 0.5, 1, and 0.75, respectively. The solid lines are video-based methods with a variable keyframe interval ranging from 1 to 5. For keyframe segmentation, ours-BiSeNet-R18 and ours-SwiftNet-R19 adopt BiSeNet-R18 (0.75) and SwiftNet-R18 (0.75), respectively. Likewise, A-X39 uses BiSeNet-R18 (0.75). The mIoU is evaluated at full resolution without regard to the input scaling factor.}
        \vspace{-0.5cm}
        %\captionof{figure}{First caption}
        %\captionof{figure}{Second caption}
        \label{fig:acc_speed_int5}
    \end{figure}

==> figs/edge_error.tex <==
    \begin{figure}[ht]
        \centering
        %\setlength\tabcolsep{0.25em}
        %\captionsetup{textfont=normalfont}
        \begin{tabular}{@{}cc@{}}
        \includegraphics[width=4cm, height=2cm]{results/figures/edge/edge.png} &  \includegraphics[width=4cm, height=2cm]{results/figures/edge/error_downscale.png}\\
           (a) Edge map & (b) Error map  \\
        \end{tabular}
        \caption{Comparison between the edge map $E_t$ and the error map, which indicates the errors on the temporally warped segmentation $\hat{S}_{t}^-$.}
        \label{fig:edge_com}
    \end{figure}

==> figs/hffb.tex <==
    \begin{figure}[ht]
        \centering\footnotesize
        %\captionsetup{textfont=normalfont}
        \includegraphics[height=11cm, width=.8\linewidth]{results/component_arc/HFFB_arc.png}
        \vspace{-0.4cm}
        \caption{The architecture of our lightweight optical flow network. The red, blue, and green blocks each output 64, 32, and 2 channels, respectively. Except for the gray and green blocks, the other blocks all include $3 \times 3$ convolutional layers followed by batch normalization and LeakyReLU with a slope factor of 0.1.}
        \label{fig:hffb_arc}
        \vspace{-0.3cm}
    \end{figure}

==> figs/idk.tex <==
\begin{figure}[h]
     \centering\footnotesize
     %\captionsetup{textfont=normalfont}
     \includegraphics[width=.8\linewidth]{results/component_arc/idk_arc.png}
     \caption{Illustration of ideal-delay kernels.}
     \vspace{-0.1cm}
     \label{fig:copy_kernel}
\end{figure}

==> figs/qualitative.tex <==
\begin{figure*}[ht]
            \centering
            %\captionsetup{textfont=normalfont}
            \setlength\tabcolsep{0.18em}
            \begin{tabular}{@{}cccccc@{}}
                %\raisebox{1.75\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{k}} &
                %\includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/ours/1.png} &
                %\includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/A-X39/1.png} &
                %\includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/swnet/1.png} &
                %\includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/bisenet/1.png} &
                \\
                
                \raisebox{1.75\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{k+1}} &
                \includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/ours/2.png} &
                \includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/A-X39/2.png} &
                \includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/swnet/2.png} &
                \includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/bisenet/2.png} &
                \\
                
                \raisebox{1.75\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{k+2}} & 
                \includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/ours/3.png} &
                \includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/A-X39/3.png} &
                \includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/swnet/3.png} &
                \includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/bisenet/3.png} &
                \\
                
                \raisebox{1.75\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{k+3}} & \includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/ours/4.png} &
                \includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/A-X39/4.png} &
                \includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/swnet/4.png} &
                \includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/bisenet/4.png} &
                \includegraphics[width=0.19\linewidth]{results/figures/qualitative_result/325/GT.png} \\
                &(a) Ours-SwiftNet (0.75) & (b) A-Lite & (c) SwiftNet-R18 (0.5) & (d) BiSeNet-R18 (0.5) & (e) Ground Truth \\    
            \end{tabular}
            \caption{Qualitative evaluation. From top to bottom, each row with index k + n shows the segmentation results for a video frame that is n steps after the keyframe k. Note that only the last frame k+3 has the ground-truth segmentation. A-Lite (instead of A-X39) is used for comparison as it is the only version of Accel that achieves a similar throughput to the others.}
            \label{fig:qualitative_single_image}
        \end{figure*}     

==> tables/IDK.tex <==
    \begin{table}[t]
        \centering
        \setlength{\tabcolsep}{5pt}
        %\captionsetup{textfont=normalfont}
        \begin{tabular}{p{0.2\linewidth}p{0.2\linewidth}ccccc}
            \hline
             & & \multicolumn{5}{c}{Keyframe interval} \\ \cline{3-7}
            Metric & Scheme & 1 & 2 & 3 & 4 & 5 \\ \hline
            Avg. & IDK & 74.4 & 73.7 & 72.6 & 71.8 & 70.9 \\ 
            %  & RI+TK & 74.4 & 73.6 & 72.5 & 71.6 & 70.6 \\
            mIoU ($\%$) & IDK+Finetune & 74.4 & 73.6 & 72.6 & 71.8 & 70.9 \\
            \hline
        \end{tabular}
        \vspace{0.5em}
        \caption{Accuracy comparison between models with ideal-delay kernels and fine-tuned kernels for various keyframe intervals. \textbf{IDK:} Ideal-delay Kernel.}
        \label{table:set_com}
    \end{table}

==> tables/IDK_size.tex <==
    \begin{table}[t]
        %\centering\footnotesize
        \setlength{\tabcolsep}{6pt}
        %\captionsetup{textfont=normalfont}
        \begin{tabular}{p{0.2\linewidth}p{0.2\linewidth}|ccc}
            \hline
            Kernel & $\#$ of & Avg.  & Min. & FPS \\ 
            size & filters & mIoU ($\%$) & mIoU ($\%$) \\ \hline
            3 $\times$ 3 &  9 & 70.9 & 67.7 & 155 \\
            %3 $\times$ 3 & 17 & 70.9 & 67.6 & 148 \\
            %5 $\times$ 5 &  9 & 71.0 & 67.7 & 151 \\
            5 $\times$ 5 & 17 & 71.1 & 67.9 & 144 \\
            %7 $\times$ 7 &  9 & 71.0 & 67.8 & 146 \\
            %7 $\times$ 7 & 17 & 71.1 & 68.0 & 140 \\
            \hline
        \end{tabular}
        \vspace{0.5em}
        \caption{Impact of the size of the ideal-delay kernels on accuracy and throughput. The mIoU is measured at the keyframe interval of 5.}
        \label{table:com_kernel_size}
    \end{table}

==> tables/bk_speed.tex <==
\begin{figure}
        \centering
        \begin{tikzpicture}
        \begin{axis}[
            height=5cm,
            width=.8\linewidth,
            xbar stacked,
            xmajorgrids,
            xminorgrids,
            minor x tick num=4,
            xmin=0,
        	bar width=15pt,
            enlarge y limits=0.2,
            legend style={at={(-0.45, 1.3)},
              anchor=north west,legend columns=2, draw=none},
            legend cell align={left},
            xlabel={Time (ms)},
            symbolic y coords={{Ours-SwiftNet-R18},A-X39,{SwiftNet-R18 (0.75)},{BiSeNet-R18 (0.75)},BiSeNet-X39},
            ytick=data,
            major grid style={solid, black},
            ]
        \addplot+[purple2,xbar] plot coordinates {(1.1,{Ours-SwiftNet-R18})(3.8,A-X39)(0,{SwiftNet-R18 (0.75)})(0,{BiSeNet-R18 (0.75)})(0,BiSeNet-X39)};
        \addlegendentry{Flow estimation}
        \addplot+[cyan,xbar] plot coordinates {(1.0,{Ours-SwiftNet-R18})(3.3,A-X39)(0,{SwiftNet-R18 (0.75)})(0,{BiSeNet-R18 (0.75)})(0,BiSeNet-X39)};
        \addlegendentry{Temporal warping}
        \addplot+[green2,xbar] plot coordinates {(0.4,{Ours-SwiftNet-R18})(10.5,A-X39)(0,{SwiftNet-R18 (0.75)})(0,{BiSeNet-R18 (0.75)})(0,BiSeNet-X39)};
        \addlegendentry{Feature extraction}
        \addplot+[orange,xbar] plot coordinates {(1.6,{Ours-SwiftNet-R18})(0.5,A-X39)(0,{SwiftNet-R18 (0.75)})(0,{BiSeNet-R18 (0.75)})(0,BiSeNet-X39)};
        \addlegendentry{Feature/Segmentation fusion}
        \addplot+[white,xbar,            postaction={
            pattern=crosshatch dots
        }] plot coordinates {(0,{Ours-SwiftNet-R18})(0,A-X39)(15.2,{SwiftNet-R18 (0.75)})(0,{BiSeNet-R18 (0.75)})(0,BiSeNet-X39)};
        \addplot+[white,xbar,postaction={
            pattern=crosshatch dots
        }] plot coordinates {(0,{Ours-SwiftNet-R18})(0,A-X39)(0,{SwiftNet-R18 (0.75)})(16,{BiSeNet-R18 (0.75)})(0,BiSeNet-X39)};
        \addplot+[white,xbar,postaction={
            pattern=crosshatch dots
        }] plot coordinates {(0,{Ours-SwiftNet-R18})(0,A-X39)(0,{SwiftNet-R18 (0.75)})(0,{BiSeNet-R18 (0.75)})(11,BiSeNet-X39)};
        \end{axis}
        \end{tikzpicture}
        \caption{A breakdown analysis of inference runtime.}
        \label{fig:bk_speed}
    \end{figure}

==> tables/com_kernel_size.tex <==
\begin{table}[t]
        %\centering\footnotesize
        \setlength{\tabcolsep}{6pt}
        %\captionsetup{textfont=normalfont}
        \begin{tabular}{p{0.1\linewidth}p{0.2\linewidth}|ccc}
            \hline
            Kernel & $\#$ of & Avg.  & Min. & FPS \\ 
            size & filters & mIoU ($\%$) & mIoU ($\%$) \\ \hline
            3 $\times$ 3 &  9 & 70.9 & 67.7 & 155 \\
            %3 $\times$ 3 & 17 & 70.9 & 67.6 & 148 \\
            %5 $\times$ 5 &  9 & 71.0 & 67.7 & 151 \\
            5 $\times$ 5 & 17 & 71.1 & 67.9 & 144 \\
            %7 $\times$ 7 &  9 & 71.0 & 67.8 & 146 \\
            %7 $\times$ 7 & 17 & 71.1 & 68.0 & 140 \\
            \hline
        \end{tabular}
        \vspace{0.5em}
        \caption{Impact of the size of the ideal-delay kernels on accuracy and throughput. The mIoU is measured at the keyframe interval of 5.}
        \label{table:com_kernel_size}
        %\vspace{-1.0cm}
    \end{table}
